WACO: Word-Aligned Contrastive Learning for Speech Translation

End-to-end Speech Translation (E2E ST) aims to directly translate source speech into target text. Existing ST methods perform poorly when only extremely small speech-text data are available for training. We observe that an ST model's performance closely correlates with its embedding similarity between speech and source transcript. In this paper, we propose Word-Aligned COntrastive learning (WACO), a simple and effective method for extremely low-resource speech-to-text translation. Our key idea is bridging word-level representations for both speech and text modalities via contrastive learning. We evaluate WACO and other methods on the MuST-C dataset, a widely used ST benchmark, and on a low-resource direction Maltese-English from IWSLT 2023. Our experiments demonstrate that WACO outperforms the best baseline by 9+ BLEU points with only 1-hour parallel ST data. Code is available at https://github.com/owaski/WACO.

==> table/intro.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l|c} \toprule
        \textbf{Method} & \textbf{BLEU} \\\midrule
        CTC-BPE & 18.3 \\
        CTC-Phoneme & 14.3 \\
        ConST & 16.9 \\ 
        \method (ours) & \textbf{20.1} \\ \bottomrule
    \end{tabular}
    \caption{BLEU scores of cross-modal methods trained with only 100 hours of ASR data and 10 hours of ST data on MuST-C En-De corpus. \yerong{1. Add 400 hours result, to show the drop; 2. no need to show ours (not sure)}}
    \label{tab:intro}
\end{table}

\begin{table}[t]
    \centering
    \begin{tabular}{l|cc|r}
        \toprule
         & \multicolumn{2}{|c|}{\textbf{Hours of ST data}} &  \\
        \midrule
        \textbf{Method} & 400h & 10h & $\Delta$ \\
        \midrule
        ConST & 28.3 & 16.9 & - 11.4\\
        CTC-BPE & 27.6? & 18.3 & - 9.3 \\
        CTC-Phoneme & ? & 14.5 & ?\\
        \bottomrule
    \end{tabular}
    \caption{BLEU scores of cross-modal methods trained with only 100 hours of ASR data and 10 hours of ST data on MuST-C En-De corpus. ConST~\cite{ye-etal-2022-cross} bridges the sentence-level representations of two modalities by adopting contrastive learning approach. CTC models the alignment between speech and transcription, and based on the different granularity of the transcribed texts (i.e., tokenization), we consider two common variants: Byte-Pair Encoding and Phoneme, noted as CTC-BPE and CTC-Phoneme.}
    \label{tab:my_label}
\end{table}

==> table/main_mustc.tex <==
\begin{table*}[t]
% \setlength{\abovecaptionskip}{-0.cm}
% \setlength{\belowcaptionskip}{-0.5cm}
\centering
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|ccc|c}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{4}{c|}{\textbf{External Data}} & \multicolumn{9}{c}{\textbf{BLEU}} \\
    & \textbf{Speech} & \textbf{Text} & \textbf{ASR}  & \textbf{MT}  & 
    \textbf{De} & \textbf{Es} & \textbf{Fr} & \textbf{Avg.} \\ 
    \midrule
    \multicolumn{9}{c}{\emph{w/o external MT data}} \\
    \midrule
    Fairseq ST~\citep{wang2020fairseqs2t}  & - & - & - & - & 
        22.7 & 27.2 & 32.9 & ? \\
    NeurST~\cite{zhao2021neurst} & - & - & - & - & 
        22.8 & 27.4 & 33.3 & ? \\
    Espnet ST~\cite{inaguma2020espnet} & - & - & - & - & 
        22.9 & 28.0 & 32.8 & ? \\
    % AFS~\cite{zhang2020adaptive} & - & - & - & - & 
    %     22.4 & 26.9 & 31.6 & 23.0 & 24.9 &26.3 & 21.0 & 14.7 & 23.9 \\
    Dual Decoder~\cite{le2020dual} & - & - & - & - & 
        23.6 &28.1 & 33.5 & ? \\
    W-Transf.~\cite{ye2021end} & \checkmark & - & - & - & 
        23.6 & 28.4 & 34.6 & ? \\
    Speechformer~\cite{papi2021speechformer}& - & - & - & - &
        23.6 & 28.5 & - & - \\
    LightweightAdaptor~\cite{le2021lightweight} & - & - & -  & -  & 
        24.7 & 28.7 & 35.0 & ? \\
    Self-training~\citep{pino2020self} & \checkmark & - &  \checkmark & - & 
        25.2 & - & 34.5 & -\\
    SATE~\cite{xu2021stacked} & - & - & - & - & 
        25.2 & - & - & -\\ 
    BiKD~\cite{inaguma2021source} & - & - & - & - & 
        25.3 & - & 35.3 & - \\
    % W2V2-Transformer(mixup) & \checkmark & - & - & - & 
        % 24.1 & 35.0 & 16.3 \\
    % W-Transf.~\cite{han2021learning} & \checkmark & - & - & - & 
    %     22.3 & 34.3 & 15.8 \\
    Mutual-learning~\cite{zhao2021mutual} & - & - & - & - & 
        - & 28.7 & 36.3 & - \\
    XSTNet~\cite{ye2021end} & \checkmark & - & - & - & 
        25.5 & 29.6 & 36.0 & - \\
    ConST & \checkmark & - & - & - & 
        25.7 & 30.4 & 36.8 & -  \\
    % Pretrain MT & - & - & \texttimes & 28.0 & 40.4 & 18.8 & 33.4 & 29.1 & 26.6 & 34.0 & 33.5 \\
    
    \midrule
    \multicolumn{9}{c}{\emph{w/ external MT data}} \\
    \midrule
    MTL~\cite{tang2021general}  & - & - & - & \checkmark  & 
        23.9 & 28.6 & 33.1 & ? \\
    FAT-ST (Big)~\cite{zheng2021fused}  & \checkmark  &\checkmark  & \checkmark  & \checkmark  & 
        25.5 & 30.8 & - & -  \\
    JT-S-MT~\cite{tang2021improving} & - & - & - & \checkmark &
        26.8 & 31.0 & 37.4 & ?\\
    Chimera~\cite{han2021learning}  & \checkmark & - & -  & \checkmark  & 
        27.1\textsuperscript{\textdagger} & 30.6 & 35.6 &  \\
    XSTNet~\cite{ye2021end} & \checkmark & - & -  & \checkmark  & 
        27.1 & 30.8 & 38.0 & ? \\
    SATE~\cite{xu2021stacked}  & - & - & \checkmark  & \checkmark  & 
        28.1\textsuperscript{\textdagger}  & - & -&-\\ 
    STEMM~\cite{fang2022stemm} & \checkmark & - & -  & \checkmark  & 
        28.7 & 31.0 & 37.4 & ? \\
    TaskAware~\cite{indurthi2021task} & - & - & \checkmark  & \checkmark  &
        \textbf{28.9}& - &- &- \\
    STPT~\cite{tang2022unified} & \checkmark & \checkmark & \checkmark  & \checkmark  &
        - & \textbf{33.1} & \textbf{39.7} & -\\
    ConST  & \checkmark & - & -  & \checkmark  &
        28.3  & 32.0 & 38.3 & - \\ 
    \textbf{\method} & \\
    \bottomrule
\end{tabular}
}
\caption{Case-sensitive detokenized BLEU scores on MuST-C \texttt{tst-COMMON} set. "Speech" denotes unlabeled speech data. "Text" means unlabeled text data, \textit{e.g.} Europarl V7~\cite{koehn2005europarl}, CC25~\cite{liu2020multilingual}. \textdagger \ use external 40M OpenSubtitles~\citep{lison2016opensubtitles2016} MT data. Other models only use WMT data.
% * and ** mean the improvements over W2V2-Transformer baseline is statistically significant ($p < 0.05$ and $p < 0.01$, respectively).
}
\label{tab:main_result_vs_e2e}
\end{table*}


